BlockScope: Detecting and Investigating Propagated Vulnerabilities in Forked Blockchain Projects

Due to the open-source nature of the blockchain ecosystem, it is common for new blockchains to fork or partially reuse the code of classic blockchains. For example, the popular Dogecoin, Litecoin, Binance BSC, and Polygon are all variants of Bitcoin/Ethereum. These "forked" blockchains thus could encounter similar vulnerabilities that are propagated from Bitcoin/Ethereum during forking or subsequently commit fetching. In this paper, we conduct a systematic study of detecting and investigating the propagated vulnerabilities in forked blockchain projects. To facilitate this study, we propose BlockScope, a novel tool that can effectively and efficiently detect multiple types of cloned vulnerabilities given an input of existing Bitcoin/Ethereum security patches. Specifically, BlockScope adopts similarity-based code match and designs a new way of calculating code similarity to cover all the syntax-wide variant (i.e., Type-1, Type-2, and Type-3) clones. Moreover, BlockScope automatically extracts and leverages the contexts of patch code to narrow down the search scope and locate only potentially relevant code for comparison. Our evaluation shows that BlockScope achieves good precision and high recall both at 91.8% (1.8 times higher recall than that in ReDeBug). BlockScope allows us to discover 101 previously unknown vulnerabilities in 13 out of the 16 forked projects of Bitcoin and Ethereum, including 16 from Dogecoin, 6 from Litecoin, 1 from Binance, and 4 from Optimism. We have reported all the vulnerabilities to their developers; 40 of them have been patched or accepted, 66 were acknowledged or under pending, and only 4 were rejected. We further investigate the propagation and patching processes of discovered vulnerabilities, and reveal three types of vulnerability propagation from source to forked projects, as well as the long delay (over 200 days) for releasing patches in Bitcoin forks.

==> resources/old/fig_delay_picture.tex <==
\begin{figure*}[t!]
	\hspace{-2ex}
	\begin{adjustbox}{center}
		\parbox{1.0\textwidth}{
		    \begin{subfigure}{0.33\textwidth}
				\centering
		  		\includegraphics[width=\linewidth]{resources/repo_delay_bitcoin-abc}
				\caption{Bitcoin Cash}
				\label{fig:delay_abc}
			\end{subfigure}
			\begin{subfigure}{0.33\textwidth}
				\centering
		  		\includegraphics[width=\linewidth]{resources/repo_delay_litecoin}
				\caption{Litecoin}
				\label{fig:delay_lite}
			\end{subfigure}
			\begin{subfigure}{0.33\textwidth}
				\centering
		  		\includegraphics[width=\linewidth]{resources/repo_delay_dash}
				\caption{Dash}
				\label{fig:delay_dash}
			\end{subfigure}
			\begin{subfigure}{0.33\textwidth}
				\centering
		  		\includegraphics[width=\linewidth]{resources/repo_delay_BTCGPU}
				\caption{Bitcoin Gold}
				\label{fig:delay_gpu}
			\end{subfigure}
			\begin{subfigure}{0.33\textwidth}
				\centering
		  		\includegraphics[width=\linewidth]{resources/repo_delay_qtum}
				\caption{Qtum}
				\label{fig:delay_qtum}
			\end{subfigure}
			\begin{subfigure}{0.33\textwidth}
				\centering
		  		\includegraphics[width=\linewidth]{resources/repo_delay_digibyte}
				\caption{DigiByte}
				\label{fig:delay_digi}
			\end{subfigure}
		}
	\end{adjustbox}
    %\vspace{-2ex}
	\caption{CDF plot of \# the delay days per security patch.}
    %\vspace{-2ex}
	\label{fig:repo_delay}
\end{figure*}


==> resources/old/result.tex <==
\subsection{Vulnerability Detection Results}
\label{sec:result}


Since \name can not only detect cloned vulnerabilities but also determine whether a patch is applied, each raw output could be corresponding to one of the three possible situations: 
(i) a propagated vulnerability detected; 
(ii) the patch having been applied; 
and (iii) the context of patch code not existing in the forked project.
We present the detailed detection results of (i) in \mytab~\ref{tab:exp_compare} and (ii) in \mytab~\ref{tab:fix_result}.
Note that we do not list (iii) as it is not essential to our investigation.


As shown in \mytab~\ref{tab:exp_compare} and \mytab~\ref{tab:fix_result}, \name can detect both vulnerable and fixed cases in a high accuracy.
%In total, \name determines 103 outputs as vulnerabilities with only seven false negatives and nine false positives, which indicates that \name achieves a vulnerability coverage of 93.1\% in our dataset.
For each individual project, \name incurs at most two false positives/negatives.
Specifically, for Litecoin, Binance, Celo, and Optimism, \name detects all of the vulnerabilities without any false detection.
Moreover, for Dogecoin, Bitcoin Cash, and Qtum, \name does not generate any false negatives, while for Bitcoin Gold and DigiByte, \name does not output any false positives.
The detection result of the fixed cases is also encouraging and \name even achieves higher accuracy than that for the vulnerable cases.
The overall coverage for the fixed cases is as high as 97.8\%.
Note that according to our manual verification, \name has only one case of determining a vulnerability as fixed, which further demonstrates the robustness of \name.


% \mytab~\ref{tab:blockscope_result} presents the detailed detection results of \name.
% Each raw output could be corresponding to three possible situations:
% (i) a propagated vulnerability detected, i.e., the \red{\#Vuln} column in \mytab~\ref{tab:blockscope_result},
% (ii) the patch having been applied, i.e., the \red{\#Fixed} column,
% and (iii) the context of patch code not existed in the forked project, i.e., the \red{\#NoCode} column.
% Note that vulnerabilities in the \red{\#Vuln} column include both true positives and false negatives
% Note that the number of vulnerabilities contains both true positives and false negatives, and the false positives are either categorized into `fixed' (only one case) or `N/A' (eight cases).
% As we can see, for the 34 patches we examined, only Qtum is free of vulnerabilities and has fixed 88.2\% of the cloned vulnerabilities, while the other ten forked projects are problematic.
% Specifically, Dogecoin and Ravencoin contribute 18 and 17 vulnerabilities but only have fixed one and three vulnerabilities, respectively.
% We also notice that Bitcoin SV, Zcash, and Horizen have more than twenty N/A cases each.


%TODO
%\input{resources/tab/tab_top_commits}
%Besides the vulnerable forked projects, we also summarize the top commits that are reported as vulnerabilities in at least five projects, as shown in \mytab~\ref{tab:top_commits_vuln}.
%To our surprise, even though commits \texttt{d8318318} and \texttt{a2714a5c} have already been assigned CVEs, we still identify these two vulnerabilities in seven and five forked projects, respectively.
%Moreover, for some commits, such as \texttt{8313fa8e} and \texttt{5efcb772}, they require no more than five lines of code change yet remain unfixed in nine forked projects each.


%The result is also not optimistic when we review the Fixed Cases.
For the result of fixed cases, while Bitcoin's 11 forked projects have fixed 119 vulnerabilities, five of them, Dogecoin, Bitcoin SV, Zcash, Horizen, and Ravencoin, fixed only six vulnerabilities in total.
Specifically, Horizen did not fix any of the vulnerabilities.
The result for the other six projects seems satisfactory, as they fixed more than ten vulnerabilities each.
However, when we perform a detailed patch delay analysis on these six projects in \mysec\ref{subsec:patch_delay}, we find that it takes a long time for them to fix a vulnerability.
In extreme cases, e.g., Bitcoin Cash and Dash, the patch delay exceed 1,000 days.
These observations indicate that the developers of the forked projects are not actively following Bitcoin's security development.
The result for the five forked projects of \eth is more acceptable than Bitcoin.
Specifically, for the six investigated patches, four of the five forked projects have applied more than half of the patches each, with only Optimism fixing just one.


%TODO
%As we want to be responsible to the community and confirm the vulnerabilities in the forked projects, we reproduce the Bitcoin exploitable ones on the forked projects.
%Taken \texttt{a2714a5c} as an example, it is a case of argument injection vulnerability on the GUI program of Bitcoin.
%Specifically, the \texttt{QApplication} in Qt framework used by the GUI program will parse Qt built-in arguments, such as \texttt{-reverse} and \texttt{-platformpluginpath}.
%These arguments should be ignored, as they may introduce unexpected behaviors of the GUI program.
%The \texttt{-platformpluginpath} argument is especially dangerous since it may lead to the execution of malicious Qt plugins.
%\name identifies this vulnerability in five forked projects, and we successfully reproduce it on all of them.
%We provide a screenshot of the reversed Dogecoin GUI in \myfig~\ref{fig:doge_case}.


==> resources/old/tab_lite_example.tex <==
\begin{table}[t!]
	\centering
	\caption{The appearance of CVE-2019-15974 in Litecoin.}
	\label{tab:lite_exp}
	\vspace{-2ex}
	\begin{adjustbox}{center} %angle=90
	\scalebox{0.67}{
		\begin{tabular}{|rl|}
			\multicolumn{2}{l}{src/support/lockedpool.cpp} \\
			\hline
			244 & \texttt{\hspace{5mm}void *addr;}                    \\
			245 & \texttt{\hspace{5mm}len = align\_up(len, page\_size);}                    \\
			246 & \texttt{\hspace{5mm}addr = mmap(nullptr, len, PROT\_READ|PROT\_WRITE, ..., -1, 0);}                    \\
			247 & \texttt{\hspace{5mm}if (addr == MAP\_FAILED) \{}       \\
			248 & \texttt{\hspace{10mm}return nullptr;}                   \\
			249 & \texttt{\hspace{5mm}\}}                                \\
			250 & \texttt{\hspace{5mm}if (addr) \{}                      \\
			251 & \texttt{\hspace{10mm}*lockingSuccess = mlock(addr, len) == 0;}                                          \\
			252 & \texttt{\hspace{5mm}\}}                                \\
			253 & \texttt{\hspace{5mm}return addr;}                      \\
			254 & \texttt{\}}                                \\ \hline
			\multicolumn{2}{l}{\hspace*{123mm}} \\
		\end{tabular}%
	}
	\end{adjustbox}
	\vspace{-2ex}
\end{table}


==> resources/old/tab_patch_outdated.tex <==
\begin{table}[h!]
    \centering
	\caption{The outdated patch.}
	\label{tab:patch_oudated}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{Code of Bitcoin PR\#13808}
            \label{tab:PR13808}
            \vspace{-2ex}
            \scalebox{0.55}{
                \begin{tabular}{llcl}
                \multicolumn{4}{l}{\hspace*{150mm}} \\ \hline
                \rowcolor[HTML]{EDF5FF}
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}18f690ec2f7eb1b4aa51825bfed0cbfdadc93ac7 - src/wallet/wallet.cpp}                                                                                                                                                                                                                    \\
                \rowcolor[HTML]{EDF5FF}
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2525,6 +2527,12 @@ \texttt{bool CWallet::SelectCoins(const std::vector\& vAvailableCoins, const CAm}}                                                                                                                                            \\ \hline
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2525,6 +2527,12 @@ \texttt{bool CWallet::SelectCoins(...)}}                                                                                                                                            \\ \hline
                \rowcolor[HTML]{FFFFFF}
                {\color[HTML]{24292F} 2525} & {\color[HTML]{24292F} 2527} & {\color[HTML]{24292F} }                                             & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} }                                                                                                                                               \\
                \rowcolor[HTML]{FFFFFF}
                {\color[HTML]{24292F} 2526} & {\color[HTML]{24292F} 2528} & {\color[HTML]{24292F} }                                             & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{// form groups from remaining coins; note that preset coins will not}}                                                                           \\
                \rowcolor[HTML]{FFFFFF}
                {\color[HTML]{24292F} 2527} & {\color[HTML]{24292F} 2529} & {\color[HTML]{24292F} }                                             & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{// automatically have their associated (same address) coins included}}                                                                           \\
                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{24292F} }     & {\color[HTML]{24292F} 2530} & {\color[HTML]{24292F} +}                                            & {\color[HTML]{24292F} \texttt{if (coin\_control.m\_avoid\_partial\_spends \&\& vCoins.size() \textgreater OUTPUT\_GROUP\_MAX\_ENTRIES) \{}}                                                            \\
                {\color[HTML]{24292F} }     & {\color[HTML]{24292F} 2530} & {\color[HTML]{24292F} +}                                            & {\color[HTML]{24292F} \texttt{if (... \&\& vCoins.size() \textgreater OUTPUT\_GROUP\_MAX\_ENTRIES) \{}}                                                            \\
                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }     & {\color[HTML]{24292F} 2531} & {\color[HTML]{24292F} +}                                            & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{// Cases where we have 11+ outputs all pointing to the same destination may result in}}                                                          \\
                {\color[HTML]{CDFFCC} }     & {\color[HTML]{24292F} 2531} & {\color[HTML]{24292F} +}                                            & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{\hspace{5mm}// Cases where we have 11+ outputs all pointing to ...}}                                                          \\
                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{24292F} }     & {\color[HTML]{24292F} 2532} & {\color[HTML]{24292F} +}                                            & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{// privacy leaks as they will potentially be deterministically sorted. We solve that by}}                                                        \\
                {\color[HTML]{24292F} }     & {\color[HTML]{24292F} 2532} & {\color[HTML]{24292F} +}                                            & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{\hspace{5mm}// privacy leaks as they will potentially be ...}}                                                        \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{24292F} }     & {\color[HTML]{24292F} 2533} & {\color[HTML]{24292F} +}                                            & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{\hspace{5mm}// explicitly shuffling the outputs before processing}}                                                                                          \\
                \rowcolor[HTML]{CDFFCC}
                                            & {\color[HTML]{24292F} 2534} & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}+}                       & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{\hspace{5mm}std::shuffle(vCoins.begin(), vCoins.end(), FastRandomContext());}}                                                                               \\
                \rowcolor[HTML]{CDFFCC}
                                            & {\color[HTML]{24292F} 2535} & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}+}                       & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{\}}}                                                                                                                                             \\
                \rowcolor[HTML]{FFFFFF}
%                2538                        & {\color[HTML]{24292F} 2536} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}                        & {\color[HTML]{24292F} \texttt{std::vector\textless{}OutputGroup\textgreater groups = GroupOutputs(vCoins, !coin\_control.m\_avoid\_partial\_spends);}}                                                 \\
                2538                        & {\color[HTML]{24292F} 2536} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}                        & {\color[HTML]{24292F} \texttt{std::vector\textless{}OutputGroup\textgreater groups = GroupOutputs(...);}}                                                 \\
                2539                        & 2537                        & \multicolumn{1}{l}{}                                                & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} }                                                                                                                                               \\
                \rowcolor[HTML]{FFFFFF}
%                {\color[HTML]{24292F} 2530} & {\color[HTML]{24292F} 2538} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} }} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{size\_t max\_ancestors = (size\_t)std::max\textless{}int64\_t\textgreater{}(1, gArgs.GetArg("-limitancestorcount", DEFAULT\_ANCESTOR\_LIMIT));}} \\ \hline
                {\color[HTML]{24292F} 2530} & {\color[HTML]{24292F} 2538} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} }} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{size\_t max\_ancestors = (size\_t)std::max\textless{}int64\_t\textgreater{}(1, ...));}} \\ \hline
                \rowcolor[HTML]{EDF5FF}
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}{\color[HTML]{24292F} @@ -4444,7 +4452,7 @@ \texttt{std::vector CWallet::GroupOutputs(const std::vector\& outpu}}} \\ \hline
                \end{tabular}
            }
            \centering
        \end{subtable}
    \end{minipage}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{Shuffle function introduction in Bitcoin PR\#14624}
            \label{tab:intro_PR14624}
            \vspace{-2ex}
            \scalebox{0.55}{
                \begin{tabular}{
                >{\columncolor[HTML]{CDFFCC}}l
                >{\columncolor[HTML]{CDFFCC}}l
                >{\columncolor[HTML]{CDFFCC}}c
                >{\columncolor[HTML]{CDFFCC}}l }
                \multicolumn{4}{l}{\hspace*{150mm}} \\ \hline
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}e414486d56b9f06af7aeb07ce13e3c3780c2b69b - src/random.h}                                                                                                         \\
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -130,6 +138,29 @@ \texttt{class FastRandomContext \{}}                                                                                                 \\ \hline
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 151} & {\color[HTML]{24292F} }                                             & {\color[HTML]{24292F} \texttt{template\textless{}typename I, typename R\textgreater{}}} \\
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 152} & {\color[HTML]{24292F} }                                             & {\color[HTML]{24292F} \texttt{void Shuffle(I first, I last, R\&\& rng)} }               \\
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 153} & {\color[HTML]{24292F} }                                             & {\color[HTML]{24292F} \texttt{\{}}                                                      \\
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 154} & {\color[HTML]{24292F} }                                             & {\color[HTML]{24292F} \texttt{\hspace{5mm}while (first != last) \{}}                                \\
                {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 155} & {\color[HTML]{24292F} }                                             & {\color[HTML]{24292F} \texttt{\hspace{10mm}size\_t j = rng.randrange(last - first);}}                \\
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 156} & {\color[HTML]{24292F} }                                             & {\color[HTML]{24292F} \texttt{\hspace{10mm}if (j) \{}}                                               \\
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 157} & {\color[HTML]{24292F} }                                             & {\color[HTML]{24292F} \texttt{\hspace{15mm}using std::swap;}}                                        \\
                                        & {\color[HTML]{24292F} 158} & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}}                        & {\color[HTML]{24292F} \texttt{\hspace{15mm}swap(*first, *(first + j));}}                             \\
                                        & {\color[HTML]{24292F} 159} & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}}                        & {\color[HTML]{24292F} \texttt{\hspace{10mm}\}}}                                                      \\
                                        & {\color[HTML]{24292F} 160} & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}}                        & {\color[HTML]{24292F} \texttt{\hspace{10mm}++first;}}                                                \\
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 161} & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} }} & {\color[HTML]{24292F} \texttt{\hspace{5mm}\}}}                                                      \\
                {\color[HTML]{24292F} } & {\color[HTML]{24292F} 162} & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} }} & {\color[HTML]{24292F} \texttt{\}}} \\ \hline
                \end{tabular}
            }
            \centering
        \end{subtable}
    \end{minipage}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{Shuffle function usage in Bitcoin PR\#14624}
            \label{tab:usage_PR14624}
            \centering
            \vspace{-2ex}
            \scalebox{0.55}{
                \begin{tabular}{llcl}
                \multicolumn{4}{l}{\hspace*{150mm}} \\ \hline
                \rowcolor[HTML]{EDF5FF}
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}e414486d56b9f06af7aeb07ce13e3c3780c2b69b - src/wallet/wallet.cpp}                                                                                                                                          \\
                \rowcolor[HTML]{EDF5FF}
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2462,7 +2462,7 @@ \texttt{bool CWallet::SelectCoins(const std::vector\& vAvailableCoins, const CAm}}                                                                                            \\ \hline
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2462,7 +2462,7 @@ \texttt{bool CWallet::SelectCoins(const std::vector\& ...}}                                                                                            \\ \hline
                \rowcolor[HTML]{FFFFFF}
%                {\color[HTML]{24292F} 1896} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} 1896} & {\color[HTML]{24292F} }  & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{// Cases where we have 11+ outputs all pointing to the same destination may result in}}   \\
                {\color[HTML]{24292F} 2462} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} 2462} & {\color[HTML]{24292F} }  & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{\hspace{5mm}// Cases where we have 11+ outputs all pointing to ...}}   \\
                \rowcolor[HTML]{FFFFFF}
%                {\color[HTML]{24292F} 1897} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} 1897} & {\color[HTML]{24292F} }  & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{// privacy leaks as they will potentially be deterministically sorted. We solve that by}} \\
                {\color[HTML]{24292F} 2463} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} 2463} & {\color[HTML]{24292F} }  & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{\hspace{5mm}// privacy leaks as they will potentially ...}} \\
                \rowcolor[HTML]{FFFFFF}
                {\color[HTML]{24292F} 2464} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} 2464} & {\color[HTML]{24292F} }  & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{\hspace{5mm}// explicitly shuffling the outputs before processing}}                                   \\
                \rowcolor[HTML]{FFDDDB}
                {\color[HTML]{24292F} 2465} & {\color[HTML]{24292F} }                             & {\color[HTML]{24292F} -} & {\color[HTML]{24292F} \texttt{\hspace{5mm}std::shuffle(vCoins.begin(), vCoins.end(), FastRandomContext());}}                                                \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{CDFFCC} }     & {\color[HTML]{24292F} 2465}                         & {\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{\hspace{5mm}Shuffle(vCoins.begin(), vCoins.end(), FastRandomContext());}}                                                     \\
                \rowcolor[HTML]{FFFFFF}
                {\color[HTML]{24292F} 2466} & {\color[HTML]{24292F} 2466}                         & {\color[HTML]{24292F} }  & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{\}}}                                                                                      \\
                \rowcolor[HTML]{FFFFFF}
%                {\color[HTML]{24292F} 1901} & {\color[HTML]{24292F} 1891}                         & {\color[HTML]{24292F} }  & {\color[HTML]{24292F} \texttt{std::vector groups = GroupOutputs(vCoins, !coin\_control.m\_avoid\_partial\_spends);}}                 \\ \hline
                {\color[HTML]{24292F} 2467} & {\color[HTML]{24292F} 2467}                         & {\color[HTML]{24292F} }  & {\color[HTML]{24292F} \texttt{std::vector groups = GroupOutputs(...);}}                 \\ \hline
                \rowcolor[HTML]{EDF5FF}
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}{\color[HTML]{24292F} @@ -2922,7 +2922,7 @@ \texttt{bool CWallet::CreateTransaction(interfaces::Chain::Lock\& locked\_chain, const std}}} \\ \hline
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}{\color[HTML]{24292F} @@ -2922,7 +2922,7 @@ \texttt{bool CWallet::CreateTransaction(...}}} \\ \hline
                \end{tabular}
            }
        \end{subtable}
    \end{minipage}

%    \begin{minipage}[b]{.5\textwidth}
%        \begin{subtable}{\textwidth}
%            \caption{Bitcoin PR#12561}
%            \label{tab:PR#12561}
%            \scalebox{0.55}{
%
%            }
%            \centering
%        \end{subtable}
%    \end{minipage}


\end{table}

==> resources/old/tab_raven_example.tex <==
\begin{table}[t!]
	\centering
	\caption{The appearance of CVE-2018-17145 in Ravencoin.}
	\label{tab:raven_exp}
	\vspace{-2ex}
	\begin{adjustbox}{center} %angle=90
	\scalebox{0.67}{
		\begin{tabular}{|rl|}
			\multicolumn{2}{l}{src/wallet/wallet.h} \\
			\hline
			1099 & \texttt{const std::string\& GetAccountName(const CScript\& scriptPubKey) const;}           \\
			1100 &                            \\
			1101 & \texttt{void Inventory(const uint256 \&hash) override}                                     \\
			1102 & \texttt{\{}                \\
			1103 & \texttt{\hspace{5mm}\{}                \\
			1104 & \texttt{\hspace{10mm}LOCK(cs\_wallet);} \\
			1105 & \texttt{\hspace{10mm}std::map<uint256, int>::iterator mi = mapRequestCount.find(hash);}                              \\
			1106 & \texttt{\hspace{10mm}if (mi != mapRequestCount.end())}                                                 \\
			1107 & \texttt{\hspace{15mm}(*mi).second++;}   \\
			1108 & \texttt{\hspace{5mm}\}}                \\
			1109 & \texttt{\}}                \\
			1110 &                            \\
			1111 & \texttt{void GetScriptForMining(std::shared\_ptr<CReserveScript> \&script); //...} \\ \hline
			\multicolumn{2}{l}{\hspace*{123mm}} \\
		\end{tabular}%
	}
	\end{adjustbox}
	\vspace{-2ex}
\end{table}


==> resources/old/tab_target_outdated.tex <==
\begin{table}[h!]
    \centering
	\caption{The outdated target code.}
	\label{tab:target_outdated}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{Code of Bitcoin PR\#15305}
            \centering
            \label{tab:PR15305}
            \vspace{-2ex}
            \scalebox{0.55}{
                \begin{tabular}{cccl}
                    \multicolumn{4}{l}{\hspace*{150mm}} \\ \hline
                    \rowcolor[HTML]{EDF5FF}
                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}4433ed0f730cfd60eeba3694ff3c283ce2c0c8ee - src/validation.cpp}                                                                                                                                        \\
                    \rowcolor[HTML]{EDF5FF}
%                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2295,7 +2295,7 @@ \texttt{bool CChainState::DisconnectTip(CValidationState\& state, const CChainParams\& cha}}                                                                            \\ \hline
                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2295,7 +2295,7 @@ \texttt{bool CChainState::DisconnectTip(...}}                                                                            \\ \hline
                    \rowcolor[HTML]{FFFFFF}
                    {\color[HTML]{24292F} 2295} & {\color[HTML]{24292F} 2295} & {\color[HTML]{24292F} }                          & {\color[HTML]{24292F} \texttt{\hspace{5mm}std::shared\_ptr\textless{}CBlock\textgreater pblock = std::make\_shared\textless{}CBlock\textgreater{}();}} \\
                    \rowcolor[HTML]{FFFFFF}
                    {\color[HTML]{24292F} 2296} & {\color[HTML]{24292F} 2296} & {\color[HTML]{24292F} }                          & {\color[HTML]{24292F} \texttt{\hspace{5mm}CBlock\& block = *pblock;}}                                                                                  \\
                    \rowcolor[HTML]{FFFFFF}
%                    {\color[HTML]{24292F} 2297} & {\color[HTML]{24292F} 2297} & {\color[HTML]{24292F} }                          & {\color[HTML]{24292F} \texttt{if (!ReadBlockFromDisk(block, pindexDelete, chainparams.GetConsensus()))}}                                   \\
                    {\color[HTML]{24292F} 2297} & {\color[HTML]{24292F} 2297} & {\color[HTML]{24292F} }                          & {\color[HTML]{24292F} \texttt{\hspace{5mm}if (!ReadBlockFromDisk(block, pindexDelete, ...))}}                                   \\
                    \rowcolor[HTML]{FFDDDB}
                    {\color[HTML]{24292F} 2298} & {\color[HTML]{24292F} }     & {\color[HTML]{24292F} -}                         & {\color[HTML]{24292F} \texttt{\hspace{10mm}return AbortNode(state, "Failed to read block");}}                                                           \\
                    \rowcolor[HTML]{CDFFCC}
                    {\color[HTML]{CDFFCC} }     & {\color[HTML]{24292F} 2298} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{10mm}return error("DisconnectTip(): Failed to read block");}}                                                     \\
                    \rowcolor[HTML]{FFFFFF}
                    {\color[HTML]{24292F} 2299} & {\color[HTML]{24292F} 2299} & {\color[HTML]{24292F} }                          & {\color[HTML]{24292F} \texttt{\hspace{5mm}// Apply the block atomically to the chain state.}}                                                          \\
                    \rowcolor[HTML]{FFFFFF}
                    {\color[HTML]{24292F} 2300} & {\color[HTML]{24292F} 2300} & {\color[HTML]{24292F} }                          & {\color[HTML]{24292F} \texttt{\hspace{5mm}int64\_t nStart = GetTimeMicros();}}                                                                         \\
                    \rowcolor[HTML]{FFFFFF}
                    {\color[HTML]{24292F} 2301} & {\color[HTML]{24292F} 2301} &                                                  & {\color[HTML]{24292F} \texttt{\hspace{5mm}\texttt{\{}}}                                                                                        \\ \hline
                    \rowcolor[HTML]{EDF5FF}
%                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2551,6 +2551,11 @@ \texttt{bool CChainState::ActivateBestChainStep(CValidationState\& state, const CChainPar}}                                                                            \\ \hline
                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -2551,6 +2551,11 @@ \texttt{bool CChainState::ActivateBestChainStep(...)}}                                                                            \\ \hline
                    \rowcolor[HTML]{FFFFFF}
%                    2251                        & {\color[HTML]{24292F} 2251} &                                                  & {\color[HTML]{24292F} \texttt{\hspace{15mm}// This is likely a fatal error, but keep the mempool consistent,}}                                          \\
                    2251                        & {\color[HTML]{24292F} 2251} &                                                  & {\color[HTML]{24292F} \texttt{\hspace{15mm}// This is likely a fatal error, but ...,}}                                          \\
                    \rowcolor[HTML]{FFFFFF}
%                    2552                        & 2552                        &                                                  & {\color[HTML]{24292F} \texttt{\hspace{15mm}// just in case. Only remove from the mempool in this case.}}                                                \\
                    2552                        & 2552                        &                                                  & {\color[HTML]{24292F} \texttt{\hspace{15mm}// just in case. Only remove from the ...}}                                                \\
                    \rowcolor[HTML]{FFFFFF}
                    {\color[HTML]{24292F} 2553} & {\color[HTML]{24292F} 2553} & {\color[HTML]{24292F} }                          & {\color[HTML]{24292F} \texttt{\hspace{15mm}UpdateMempoolForReorg(disconnectpool, false);}}                                                              \\
                    \rowcolor[HTML]{CDFFCC}
                                                & 2554                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} }                                                                                                           \\
                    \rowcolor[HTML]{CDFFCC}
%                                                & 2555                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{\hspace{15mm}// If we're unable to disconnect a block during normal operation,}}                                          \\
                                                & 2555                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{\hspace{15mm}// If we're unable to disconnect a block ...,}}                                          \\
                    \rowcolor[HTML]{CDFFCC}
%                                                & 2556                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{\hspace{15mm}// then that is a failure of our local system -- we should abort}}                                           \\
                                                & 2556                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{\hspace{15mm}// then that is a failure of our local system -- ...}}                                           \\
                    \rowcolor[HTML]{CDFFCC}
                                                & 2257                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{\hspace{15mm}// rather than stay on a less work chain.}}                                                                  \\
                    \rowcolor[HTML]{CDFFCC}
%                                                & 2558                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{AbortNode(state, "Failed to disconnect block; see debug.log for details");}}                                 \\
                                                & 2558                        & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{\hspace{15mm}AbortNode(state, "Failed to disconnect block; see ...");}}                                 \\
                    \rowcolor[HTML]{FFFFFF}
                                                & 2559                        &                                                  & {\color[HTML]{24292F} \texttt{\hspace{15mm}return false;}}                                                                                              \\
                    \rowcolor[HTML]{FFFFFF}
                                                & 2560                        &                                                  & {\color[HTML]{24292F} \texttt{\hspace{10mm}\}}} \\ \hline
                \end{tabular}
            }
            \centering
        \end{subtable}
    \end{minipage}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{Bitcoin SV block disconnection handle.}
            \label{tab:bitcoin_sv_disconnection}
            \centering
            \vspace{-2ex}
            \scalebox{0.55}{
                \begin{tabular}{|cl|}
                \multicolumn{2}{l}{\hspace*{150mm}} \\
                \multicolumn{2}{l}{src/validation.cpp}                                    \\ \hline
                4208 & \texttt{try}                                                                \\
                4209 & \texttt{\{}                                                                 \\
                4210 & \texttt{\hspace{5mm}// we are diconnecting until we reach the fork point }              \\
                4211 & \texttt{\hspace{5mm}do}                                                                 \\
                4212 & \texttt{\hspace{5mm}\{}                                                                 \\
                4213 & \texttt{\hspace{10mm}if (!DisconnectTip(config, state, \&disconnectpool, changeSet)) \{} \\
                4214 & \texttt{\hspace{15mm}// This is likely a fatal error.   }                                \\
                4215 & \texttt{\hspace{15mm}fDisconnectFailed = true;}                                         \\
                4216 & \texttt{\hspace{15mm}return;}                                                         \\
                4217 & \texttt{\hspace{10mm}\} }                                                                \\
                4218 & \texttt{\hspace{10mm}fBlocksDisconnected = true;}                                       \\
                4219 & \texttt{\hspace{5mm}\} while (needTipDisconnect());}                                    \\
                4220 & \texttt{\} }                                                                \\
                4221 & \texttt{catch( ... )}  \\ \hline
                \end{tabular}
            }
        \end{subtable}
    \end{minipage}

\end{table}


==> resources/old/tab_top_commits.tex <==
\begin{table}[t!]
	\centering
	\caption{The commits were identified as vulnerabilities with the appearance in at least five forked projects.}
	\label{tab:top_commits_vuln}
	\begin{adjustbox}{center} %angle=90
	\scalebox{0.75}{
	\begin{threeparttable}
		\begin{tabular}{|l|l|c|c|}
			\hline
			\textbf{SHA} & \textbf{Description}                                & \textbf{Source} & \textbf{\#} \\ \hline
			8313fa8e     & Fix race caused by uninitialized read               & PR \#17906      & 9                \\
			5efcb772     & Disable bloom filter to reduce DoS risk             & PR \#16152      & 9                \\
			fa48baf2     & Avoid leaking \texttt{nLockTime} fingerprint        & PR \#15039      & 8                \\
			6c10037f     & Fix data race in \texttt{InterruptRPC()}            & PR \#14993      & 8                \\
			4433ed0f     & Abort the block if unable to disconnect             & PR \#15305      & 7                \\
			d8318318*    & Avoid dumping sensitive information in core         & PR \#15600      & 6                \\
			18f690ec     & Prevent privacy leaks by shuffling coins            & PR \#13808      & 6                \\
			e254ff5d     & Limit the maximum size for locators                 & PR \#13907      & 5                \\
			a2714a5c*    & Ignore Qt built-in command line arguments           & PR \#16578      & 5                \\
			1cff3d6c     & Prevent \texttt{InvBlock}-related attacks by random & PR \#14897      & 5                \\ \hline
		\end{tabular}%
	\begin{tablenotes}
    \item \small *: These commits are patches for the CVEs listed in \mytab\ref{tab:patch_exp}
    \end{tablenotes}
	\end{threeparttable}
	}
	\end{adjustbox}
\end{table}


% \begin{table}[t!]
% 	\centering
% 	\caption{The commits were identified as fixed with the appearance in at least five forked projects.}
% 	\label{tab:top_commits_fix}
% 	\begin{adjustbox}{center} %angle=90
% 	\scalebox{0.75}{
% 	\begin{threeparttable}
% 		\begin{tabular}{|l|l|c|c|}
% 			\hline
% 			\textbf{SHA} & \textbf{Description}                                & \textbf{Source} & \textbf{\#} \\ \hline
% 			b7b36dec     & Fix uninitialized read about \texttt{addrLocal}     & PR \#14728      & 7           \\
% 			76f74811     & Add timeout for header synchronization              & PR \#10345      & 7           \\
% 			015a5258     & Check new header not from invalid block             & PR \#11531      & 7           \\
% 			e254ff5d     & Limit the maximum size for locators                 & PR \#13907      & 6           \\
% 			fad231ad     & Merge of global unknown data in PSBTs               & PR \#13721      & 5           \\
% 			beef7ec4*    & Fix \texttt{Inventory} out-of-memory DoS            & PR \#13622      & 5           \\
% 			a23a7f60     & Avoid use of uninitialized value \texttt{bub\_used} & PR \#13546      & 5           \\
% 			37886d5e     & Disconnect outbound peers on invalid chain          & PR \#11568      & 5           \\
% 			2fb9c1e6     & Shuffle tx inputs to avoid fingerprinting           & PR \#12699      & 5           \\
% 			27ee53c1     & Check return value of \texttt{ParseUInt32()}        & PR \#13712      & 5           \\
% 			18f690ec     & Prevent privacy leaks by shuffling coins            & PR \#13808      & 5           \\ \hline
% 		\end{tabular}%
% 	\begin{tablenotes}
%     \item \small *: These commits are patches for the CVEs listed in \mytab\ref{tab:patch_exp}
%     \end{tablenotes}
% 	\end{threeparttable}
% 	}
% 	\end{adjustbox}
% \end{table}


==> resources/old/tab_vuln_root_cause.tex <==
\begin{table}[h!]
    \centering
	\caption{The root causes of the vulnerabilities.}
	\label{tab:vuln_root_cause}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{CVE-2021-3401 introduction}
            \label{tab:cve_2021_3401_intro}
            \vspace{-2ex}
            \centering
            \scalebox{0.55}{
                \begin{tabular}{
                    >{\columncolor[HTML]{CDFFCC}}l
                    >{\columncolor[HTML]{CDFFCC}}l
                    >{\columncolor[HTML]{CDFFCC}}c
                    >{\columncolor[HTML]{CDFFCC}}l }
                    \multicolumn{4}{l}{\hspace*{150mm}} \\                    \hline
%                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}src/qt/bitcoin.cpp}                                                                                                                                    \\
%                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -162,6 +158,265 @@ \texttt{void DebugMessageHandler(QtMsgType type, const QMessageLogContext\& context, cons)}}                                                                             \\ \hline
                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}202d853bbea8ecb2164b9c9dc69e2129b45f05f8 - src/qt/bitcoin.cpp}                                                                                                              \\
                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -162,6 +158,265 @@ \texttt{void DebugMessageHandler(...)}}                                                                             \\ \hline
                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 276} & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{BitcoinApplication::BitcoinApplication(int \&argc, char **argv):}} \\
%                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 276} & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} +} & {\color[HTML]{24292F} \texttt{BitcoinApplication::BitcoinApplication(int \&argc, ...):}} \\
                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 277} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}QApplication(argc, argv),}}                                        \\
                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 278} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}coreThread(0),}}                                                   \\
                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 279} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}paymentServer(0),}}                                                \\
                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 280} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}optionsModel(0),}}                                                 \\
                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 281} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}clientModel(0),}}                                                  \\
%                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 282} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}window(0),}}                                                       \\
%                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 283} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}walletModel(0),}}                                                  \\
%                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 284} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}returnValue(0)}}                                                   \\
%                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 285} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\{}}                                                               \\
%                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 286} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}setQuitOnLastWindowClosed(false);}}                                \\
%                    {\color[HTML]{CDFFCC} } & {\color[HTML]{24292F} 287} & {\color[HTML]{24292F} +}                         & {\color[HTML]{24292F} \texttt{\hspace{5mm}startThread();}}                                                   \\
                    {\color[HTML]{000000} } & {\color[HTML]{000000} 288} & \cellcolor[HTML]{CDFFCC}{\color[HTML]{000000} }  & \cellcolor[HTML]{CDFFCC}{\color[HTML]{24292F} \texttt{\}}} \\ \hline
                \end{tabular}
            }
        \end{subtable}
    \end{minipage}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{Code of Bitcoin PR\#16512}
            \label{tab:PR16512}
            \vspace{-2ex}
            \centering
            \scalebox{0.55}{
                \begin{tabular}{llcl}
                \multicolumn{4}{l}{\hspace*{150mm}} \\
                \hline
                \rowcolor[HTML]{EDF5FF}
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}6f405a1d3b38395e35571b68aae55cae50e0762a - src/rpc/rawtransaction.cpp}                                                                                                                                                                                          \\
                \rowcolor[HTML]{EDF5FF}
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}}                                                                                                                                                                                                        \\
                \rowcolor[HTML]{EDF5FF}
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -1604,8 +1605,30 @@ \texttt{UniValue joinpsbts(const JSONRPCRequest\& request)}}                                                                                                                                                         \\ \hline
                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -1604,8 +1605,30 @@ \texttt{UniValue joinpsbts(const JSONRPCRequest\& ...)}}                                                                                                                                                         \\ \hline
                \rowcolor[HTML]{FFFFFF}
%                \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}1604} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}1605} &                                              & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{merged\_psbt.unknown.insert(psbt.unknown.begin(), psbt.unknown.end());}}    \\
%                \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}1604} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}1605} &                                              & \cellcolor[HTML]{FFFFFF}{\color[HTML]{24292F} \texttt{\hspace{10mm}merged\_psbt.unknown.insert(psbt.unknown.begin(), ...}}    \\
%                \rowcolor[HTML]{FFFFFF}
%                1605                                             & 1606                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & {\color[HTML]{24292F} \texttt{\hspace{5mm}\}}}                                                                                                \\
%                \rowcolor[HTML]{FFFFFF}
%                1606                                             & 1607                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                                                          \\
%                \rowcolor[HTML]{CDFFCC}
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1608}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{// Generate list of shuffled indices for shuffling inputs and outputs of the merged PSBT}}          \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1608}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}// Generate list of shuffled indices for ...}}          \\
%                \rowcolor[HTML]{CDFFCC}
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1609}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{std::vector\textless{}int\textgreater input\_indices(merged\_psbt.inputs.size());}}                 \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1609}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}std::vector\textless{}int\textgreater input\_indices(...);}}                 \\
%                \rowcolor[HTML]{CDFFCC}
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1610}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{std::iota(input\_indices.begin(), input\_indices.end(), 0);}}                                       \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1610}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}std::iota(...);}}                                       \\
%                \rowcolor[HTML]{CDFFCC}
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1611}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{std::vector\textless{}int\textgreater output\_indices(merged\_psbt.outputs.size());}}               \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1611}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}std::vector\textless{}int\textgreater output\_indices(...);}}               \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1612}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}std::iota(output\_indices.begin(), output\_indices.end(), 0);}}                                     \\
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1612}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}std::iota(...);}}                                     \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1613}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} }                                                                                                  \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1614}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}// Shuffle input and output indicies lists}}                                                        \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1615}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}Shuffle(input\_indices.begin(), input\_indices.end(), ...);}}                       \\
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1615}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{Shuffle(input\_indices.begin(), input\_indices.end(), FastRandomContext());}}                       \\
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1615}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}Shuffle(...);}}                       \\
%                \rowcolor[HTML]{CDFFCC}
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1616}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{Shuffle(output\_indices.begin(), output\_indices.end(), FastRandomContext());}}                     \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1616}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}Shuffle(output\_indices.begin(), output\_indices.end(), ...);}}                     \\
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1616}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}Shuffle(...);}}                     \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1617}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} }                                                                                                  \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1618}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}PartiallySignedTransaction shuffled\_psbt;}}                                                        \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1619}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.tx = CMutableTransaction();}}                                                        \\
%                \rowcolor[HTML]{CDFFCC}
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1620}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{shuffled\_psbt.tx-\textgreater{}nVersion = merged\_psbt.tx-\textgreater{}nVersion;}}                \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1620}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.tx-\textgreater{}nVersion = merged\_psbt.tx-\textgreater{}nVersion;}}                \\
%%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1620}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.tx-\textgreater{}nVersion = ...;}}                \\
%                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1621}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.tx-\textgreater{}nLockTime = merged\_psbt.tx-\textgreater{}nLockTime;}}              \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1621}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.tx-\textgreater{}nLockTime = ...;}}              \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1622}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}for (int i : input\_indices) \texttt{\{}}}                                                                   \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1623}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{10mm}shuffled\_psbt.AddInput(merged\_psbt.tx-\textgreater{}vin{[}i{]}, ...);}}    \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1623}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{shuffled\_psbt.AddInput(merged\_psbt.tx-\textgreater{}vin{[}i{]}, merged\_psbt.inputs{[}i{]});}}    \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1623}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{10mm}shuffled\_psbt.AddInput(merged\_psbt.tx-\textgreater{}vin{[}i{]}, ...);}}    \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1624}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}\}}}                                                                                                \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1625}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}for (int i : output\_indices) \{}}                                                                  \\
                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1626}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{10mm}shuffled\_psbt.AddOutput(merged\_psbt.tx-\textgreater{}vout{[}i{]}, merged\_psbt.outputs{[}i{]});}} \\
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1626}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{10mm}shuffled\_psbt.AddOutput(merged\_psbt.tx-\textgreater{}vout{[}i{]}, ...);}} \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1626}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{10mm}shuffled\_psbt.AddOutput(merged\_psbt.tx-\textgreater{}vout{[}i{]}, ...);}} \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1627}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}\}}}                                                                                                \\
                \rowcolor[HTML]{CDFFCC}
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1628}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.unknown.insert(merged\_psbt.unknown.begin(), merged\_psbt.unknown.end());}}          \\
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1628}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.unknown.insert(merged\_psbt.unknown.begin(), ...);}}          \\
%                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1628}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} \texttt{\hspace{5mm}shuffled\_psbt.unknown.insert(...);}}          \\
                \rowcolor[HTML]{CDFFCC}
                {\color[HTML]{CDFFCC} }                          & {\color[HTML]{24292F} 1629}                      & {\color[HTML]{24292F} +}                     & {\color[HTML]{24292F} }                                                                                                  \\
                \rowcolor[HTML]{FFFFFF}
                1607                                             &                                                  & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} & {\color[HTML]{24292F} \texttt{\hspace{5mm}CDataStream ssTx(SER\_NETWORK, PROTOCOL\_VERSION);}}                                                \\
                \rowcolor[HTML]{FFDDDB}
                1608                                             & 1630                                             & -                                            & {\color[HTML]{24292F} \texttt{\hspace{5mm}ssTx \textless{}\textless merged\_psbt;}}                                                           \\
                \rowcolor[HTML]{CDFFCC}
                                                                 & 1631                                             & +                                            & {\color[HTML]{24292F} \texttt{\hspace{5mm}ssTx \textless{}\textless shuffled\_psbt;}}                                                         \\ \hline
                \end{tabular}
            }

        \end{subtable}
    \end{minipage}

    \begin{minipage}[b]{.5\textwidth}
        \begin{subtable}{\textwidth}
            \caption{Vulnerable variable introduction in Bitcoin}
            \label{tab:intro_vul_var}
            \vspace{-2ex}
            \centering
            \scalebox{0.55}{
                \begin{tabular}{
                        >{\columncolor[HTML]{CDFFCC}}c
                        >{\columncolor[HTML]{CDFFCC}}c
                        >{\columncolor[HTML]{CDFFCC}}c
                        >{\columncolor[HTML]{CDFFCC}}l }
                    \multicolumn{4}{l}{\hspace*{150mm}} \\  \hline
                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}08096bbbc6d6fef86943ca8ce5e6de18744d58ea - src/validation.cpp} \\
                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -79,4 +81,26 @@ \texttt{class CScheduler}}                                      \\ \hline
                    & 90   & +   & \texttt{class SingleThreadedSchedulerClient \{}                                                                    \\
                    & 91   & +   & \texttt{private:}                                                                                             \\
                    & 92   & +   & \texttt{\hspace{5mm}CScheduler *m\_pscheduler;}                                                                            \\
                    & 93   & +   &                                                                                                           \\
                    & 94   & +   & \texttt{\hspace{5mm}CCriticalSection m\_cs\_callbacks\_pending;}                                                       \\
                    & 95   & +   & \texttt{\hspace{5mm}std::list\textless{}std::function\textless{}void (void)\textgreater{}\textgreater m\_callbacks\_pending;}  \\
                    & 96   & +   & \texttt{\hspace{5mm}bool m\_are\_callbacks\_running = false; }                                                                 \\ \hline
%                    & 97   & +   & \\ \hline
                \end{tabular}
            }
        \end{subtable}
    \end{minipage}

%    \begin{minipage}[b]{.5\textwidth}
%        \begin{subtable}{\textwidth}
%            \caption{Update of CVE-2018-17144 patch in Bitcoin}
%            \label{tab:update_of_bitcoin}
%            \centering
%            \scalebox{0.55}{
%                \begin{tabular}{llll}
%
%                    \multicolumn{4}{l}{\hspace*{150mm}} \\ \hline
%                    \rowcolor[HTML]{EDF5FF}
%                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}08096bbbc6d6fef86943ca8ce5e6de18744d58ea - src/scheduler.h} \\
%                    \rowcolor[HTML]{EDF5FF}
%%                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}src/scheduler.h}                          \\
%                    \rowcolor[HTML]{EDF5FF}
%                    \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -79,4 +81,26 @@ \texttt{class CScheduler}}      \\ \hline
%                    \multicolumn{4}{c}{...}                                       \\ %\hline
%                    \rowcolor[HTML]{CDFFCC}
%                        & 90    & +    & \texttt{class SingleThreadedSchedulerClient\{}                          \\
%                    \rowcolor[HTML]{CDFFCC}
%                        & 91    & +    & \texttt{private:}                                                        \\
%                    \rowcolor[HTML]{CDFFCC}
%                        & 92    & +    & \texttt{CScheduler *m\_pscheduler;}                                      \\
%                    \rowcolor[HTML]{CDFFCC}
%                        & 93    & +    &                                                                 \\
%                    \rowcolor[HTML]{CDFFCC}
%                        & 94    & +    & \texttt{CCriticalSection m\_cs\_callbacks\_pending;}                     \\
%                    \rowcolor[HTML]{CDFFCC}
%                        & 95    & +    & \texttt{std::list<std::function<void (void)>> m\_callbacks\_pending;}    \\
%                    \rowcolor[HTML]{CDFFCC}
%                        & 96    & +    & \texttt{bool m\_are\_callbacks\_running = false;}                        \\
%                    \multicolumn{4}{c}{...} \\ \hline
%                \end{tabular}
%            }
%        \end{subtable}
%    \end{minipage}
%
%    \begin{minipage}[b]{.5\textwidth}
%        \begin{subtable}{\textwidth}
%            \caption{\texttt{CheckTransaction} function change in Ravencoin}
%            \label{tab:change_of_ravencoin}
%            \centering
%            \scalebox{0.55}{
%                \begin{tabular}{llcl}
%                \multicolumn{4}{l}{\hspace*{150mm}} \\ \hline
%                \rowcolor[HTML]{EDF5FF}
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}{\color[HTML]{24292F} }}                                                                                                        \\
%                \rowcolor[HTML]{EDF5FF}
%                \multicolumn{4}{l}{\multirow{-2}{*}{\cellcolor[HTML]{EDF5FF}{\color[HTML]{24292F} 79d71da77be1653c0640a8f5843000475020bb5c - src/validation.cpp}}}                                              \\
%                \rowcolor[HTML]{EDF5FF}
%%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}{\color[HTML]{333333} @@ -157,7 +160,7 @@ \texttt{int64\_t GetTransactionSigOpCost(const CTransaction\& tx, const CCoinsViewCache\& i}}} \\
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}{\color[HTML]{333333} @@ -157,7 +160,7 @@ \texttt{int64\_t GetTransactionSigOpCost(const CTransaction\& tx, ...}}} \\ \hline
%                157          & 160          &                                                      & \texttt{return nSigOps;}                                                                       \\
%                158          & 161          &                                                      & \}                                                                                    \\
%                159          & 162          &                                                      &                                                                                       \\
%                \rowcolor[HTML]{FFCCC9}
%                160          &              & -                                                    & \texttt{bool CheckTransaction(const CTransaction\& tx, }        \\
%                \rowcolor[HTML]{FFDDDB}
%                             &              & \multicolumn{1}{l}{\cellcolor[HTML]{FFDDDB}}         & \texttt{CValidationState \&state, bool fCheckDuplicateInputs)}                                                                \\
%                \rowcolor[HTML]{CDFFCC}
%                             & 163          & +                                                    & \texttt{bool CheckTransaction(const CTransaction\& tx, CValidationState \&state,}         \\
%                \rowcolor[HTML]{CDFFCC}
%                             &              & \multicolumn{1}{l}{\cellcolor[HTML]{CDFFCC}}         & \texttt{bool CheckDuplicateInputs, bool fMemPoolCheck)    }                                         \\
%                161          & 164          &                                                      &                                                                                       \\
%                162          & 166          &                                                      & \texttt{// Basic checks that don't depend on any context   }                                   \\
%                163          & 166          &                                                      & \texttt{if (tx.vin.empty())   }                                                                \\ \hline
%                \rowcolor[HTML]{EDF5FF}
%%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -203,6 +206,19 @@ \texttt{bool CheckTransaction(const CTransaction\& tx, CValidationState \&state, bool fChe}}
%                \multicolumn{4}{l}{\cellcolor[HTML]{EDF5FF}@@ -203,6 +206,19 @@ \texttt{bool CheckTransaction(const CTransaction\& tx, CValidationState ...}} \\                 \hline
%                \end{tabular}
%            }
%        \end{subtable}
%    \end{minipage}

%    \begin{minipage}[b]{.5\textwidth}
%        \begin{subtable}{\textwidth}
%            \caption{Bitcoin PR#12561}
%            \label{tab:PR#12561}
%            \scalebox{0.55}{
%
%            }
%            \centering
%        \end{subtable}
%    \end{minipage}
%
\end{table}

==> resources/tab/tab_patch_example.tex <==
\begin{table}[t!]
	\centering
    \caption{Different patch code examples and their contexts. \red{multiple situations?}}
	\label{tab:patch_exp}
	% \vspace{-2.5ex}
	% \begin{minipage}[b]{0.5\textwidth}
	\vspace{-2ex}
		\begin{subtable}{1.0\linewidth}
			\centering
			\caption{The security patch for CVE-2019-15974.}
			\label{tab:exp_add}
			\vspace{-3ex}
			\begin{adjustbox}{center} %angle=90
			\scalebox{0.85}{
				\begin{tabular}{ccl}
					\multicolumn{3}{l}{\hspace*{98mm}} \\
					\hline
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF}d831831822885717e9841f1ff67c19add566fa45 - src/support/lockedpool.cpp} \\
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF} \texttt{void *PosixLockedPageAllocator::AllocateLocked(size\_t ...)}} \\ \hline
					1  &    & \texttt{\hspace{5mm}void *addr;}                              \\
					2  &    & \texttt{\hspace{5mm}len = align\_up(len, page\_size);}                              \\
					3          &           & \texttt{\hspace{5mm}addr = mmap(nullptr, len, PROT\_READ|PROT\_WRITE, ...);}         \\
					4  &    & \texttt{\hspace{5mm}if (addr) \{}                              \\
					5  &    & \texttt{\hspace{10mm}*lockingSuccess = \darkred{\textbf{mlock}}(addr, len) == 0;}  \\
					\rowcolor[HTML]{CDFFCC} 
					6  & +  & \texttt{\#ifdef MADV\_DONTDUMP}                    \\
					\rowcolor[HTML]{CDFFCC}
					7  & +  & \texttt{\hspace{10mm}madvise(addr, len, MADV\_DONTDUMP);}       \\
					\rowcolor[HTML]{CDFFCC} 
					8  & +  & \texttt{\#endif}                                   \\
					9  &    & \texttt{\hspace{5mm}\}}                                        \\
					10  &    & \texttt{\hspace{5mm}return addr;}                              \\
					11  &    & \texttt{\}}                                        \\ \hline
					\multicolumn{3}{l}{\textbf{Extracted Patch Context}}                                                  \\ \hline
					\multicolumn{2}{r}{TYPE:}     & \texttt{ADD} \\
					%\multicolumn{2}{r}{ADD:}  & \multicolumn{2}{l}{(\texttt{madvise}, 254, (253, 255))}                                              \\
					\multicolumn{2}{r}{UP:} & (\texttt{mlock}, 252) \\ \hline
				\end{tabular}%
			}
			\end{adjustbox}
			\vspace{1ex}
		\end{subtable}
		\vfill
		\begin{subtable}{1.0\linewidth}
			\centering
			\caption{The security patch for CVE-2018-17145.}
			\label{tab:exp_del}
			\vspace{-3ex}
			\begin{adjustbox}{center} %angle=90
			\scalebox{0.85}{
				\begin{tabular}{ccl}
					\multicolumn{3}{l}{\hspace*{98mm}} \\
					\hline
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF}beef7ec4be725beea870a2da510d2817487601ec - src/wallet/wallet.h} \\
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF} \texttt{class CWallet final : public CCryptoKeyStore, public ...}} \\ \hline
					1  &   & \texttt{const std::string\& \darkred{\textbf{GetLabelName}}(const CScript\& ...) const;} \\
					2  &   &                                                                              \\
					\rowcolor[HTML]{FFDDDB} 
					3  & - & \texttt{void \darkred{\textbf{Inventory}}(const uint256 \&hash) override}                        \\
					\rowcolor[HTML]{FFDDDB} 
					4  & - & \texttt{\{}                                                                  \\
					\rowcolor[HTML]{FFDDDB} 
					5  & - & \texttt{\hspace{5mm}\{}                                                                  \\
					\rowcolor[HTML]{FFDDDB} 
					6  & - & \texttt{\hspace{10mm}LOCK(cs\_wallet);}                                                    \\
					\rowcolor[HTML]{FFDDDB} 
					7  & - & \texttt{\hspace{10mm}std::map<uint256, int>::iterator mi = ...;}   \\
					\rowcolor[HTML]{FFDDDB} 
					8  & - & \texttt{\hspace{10mm}if (mi != mapRequestCount.end())}                                    \\
					\rowcolor[HTML]{FFDDDB} 
					9  & - & \texttt{\hspace{15mm}(*mi).second++;}                                                     \\
					\rowcolor[HTML]{FFDDDB} 
					10 & - & \texttt{\hspace{5mm}\}}                                                                  \\
					\rowcolor[HTML]{FFDDDB} 
					11 & - & \texttt{\}}                                                                  \\
					\rowcolor[HTML]{FFDDDB} 
					12 & - &                                                                              \\
					13 &   & \texttt{void \darkred{\textbf{GetScriptForMining}}(std::shared\_ptr ... \&script);}   \\
					14 &   &                                                                              \\
					15 &   & \texttt{unsigned int GetKeyPoolSize() ...}   \\ \hline
					\multicolumn{3}{l}{\textbf{Extracted Patch Context}}                                                  \\ \hline
					\multicolumn{2}{r}{TYPE:}     & \texttt{DEL} \\
					\multicolumn{2}{r}{UP:} & (\texttt{GetLabelName}, 1065) \\
					\multicolumn{2}{r}{DOWN:} & (\texttt{GetScriptForMining}, 1077) \\ 
					\multicolumn{2}{r}{DEL:}  & (\texttt{Inventory}, 1067, (1067, 1076)) \\
                    \hline
				\end{tabular}%
			}
			\end{adjustbox}
			\vspace{1ex}
		\end{subtable}
		\vfill
		\begin{subtable}{1.0\linewidth}
			\centering
			\caption{The security patch for CVE-2021-3401.}
			\label{tab:exp_cha}
			\vspace{-3ex}
			\begin{adjustbox}{center} %angle=90
			\scalebox{0.85}{
				\begin{tabular}{ccl}
					\multicolumn{3}{l}{\hspace*{98mm}} \\
					\hline
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF}a2714a5c69f0b0506689af04c3e785f71ee0915d - src/qt/bitcoin.cpp} \\
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF} \texttt{void BitcoinCore::shutdown()}}                    \\ \hline
					1 &   & \texttt{\hspace{5mm}\}}                                         \\
					2 &   & \texttt{\}}                                         \\
					3 &   &                                                     \\
					\rowcolor[HTML]{FFDDDB} 
					4 & - & \texttt{BitcoinApplication::\darkred{\textbf{BitcoinApplication}}(interfaces ...):} \\
					\rowcolor[HTML]{FFDDDB} 
                    5 & - & \texttt{\hspace{5mm}\darkred{\textbf{QApplication}}(argc, argv),}                  \\
					\rowcolor[HTML]{CDFFCC} 
					6 & + & \texttt{static int qt\_argc = 1;}                    \\
					\rowcolor[HTML]{CDFFCC} 
					7 & + & \texttt{static const char* qt\_argv = "bitcoin-qt";} \\
					\rowcolor[HTML]{CDFFCC} 
					8 & + &                                                     \\
					\rowcolor[HTML]{CDFFCC} 
					9 & + & \texttt{BitcoinApplication::BitcoinApplication(interfaces ...}                         \\
					\rowcolor[HTML]{CDFFCC} 
					10 & + & \texttt{\hspace{5mm}QApplication(qt\_argc, const\_cast<char **>(\&qt\_argv)),}                                   \\
					11 &   & \texttt{\hspace{5mm}coreThread(nullptr),}                       \\
					12 &   & \texttt{\hspace{5mm}m\_node(node),}                              \\
					13 &   & \texttt{\hspace{5mm}optionsModel(nullptr),}                     \\ \hline
					\multicolumn{3}{l}{\textbf{Extracted Patch Context}}                                                  \\ \hline
					\multicolumn{2}{r}{TYPE:}     & \texttt{CHA} \\
					%\multicolumn{2}{r}{ADD:}  & \multicolumn{2}{l}{(\texttt{qt\_argc}, 172, (172, 176))}                                              \\
					\multicolumn{2}{r}{DEL:} & (\texttt{BitcoinApplication}, 172, (172, 173)) \\ \hline
				\end{tabular}%
			}
			\end{adjustbox}
			\vspace{1ex}
		\end{subtable}
		\vfill
		\begin{subtable}{1.0\linewidth}
			\centering
			\caption{The security patch for CVE-2022-29177.}
			\label{tab:exp_cha_1}
			\vspace{-3ex}
			\begin{adjustbox}{center} %angle=90
			\scalebox{0.85}{
				\begin{tabular}{ccl}
					\multicolumn{3}{l}{\hspace*{98mm}} \\
					\hline
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF}870b4505a05cd8b3604078ed4afcd3012bf72a47 - p2p/peer.go}             \\
					\rowcolor[HTML]{EDF5FF} 
					\multicolumn{3}{l}{\cellcolor[HTML]{EDF5FF} \texttt{func (p *Peer) handle(msg Msg) error}} \\ \hline
					1        &          & \texttt{\hspace{5mm}msg.Discard()} \\
					2        &          & \texttt{\hspace{5mm}go SendItems(p.rw, pongMsg)} \\
					3        &          & \texttt{case msg.Code == discMsg:} \\
					\rowcolor[HTML]{FFDDDB} 
					4        & -        & \texttt{\hspace{5mm}var reason [1]DiscReason} \\
					5        &          & \texttt{\hspace{5mm}// This is the last message. We don't need to ...} \\
					6        &          & \texttt{\hspace{5mm}// check errors because, the connection will be ...} \\
					\rowcolor[HTML]{FFDDDB} 
					7        & -        & \texttt{\hspace{5mm}rlp.Decode(msg.Payload, \&reason)}        \\
					\rowcolor[HTML]{FFDDDB} 
					8        & -        & \texttt{\hspace{5mm}return reason[0]}        \\
					\rowcolor[HTML]{CDFFCC} 
					9        & +        & \texttt{\hspace{5mm}var m struct\{ R DiscReason \}}         \\
					\rowcolor[HTML]{CDFFCC} 
					10        & +        & \texttt{\hspace{5mm}rlp.Decode(msg.Payload, \&m)}         \\
					\rowcolor[HTML]{CDFFCC} 
					11        & +        & \texttt{\hspace{5mm}return m.R}         \\
					12     &     & \texttt{case msg.Code < baseProtocolLength:} \\
					13     &     & \texttt{\hspace{5mm}// ignore other base protocol messages} \\
					14     &     & \texttt{\hspace{5mm}return msg.Discard()}    \\ \hline
					\multicolumn{3}{l}{\textbf{Extracted Patch Context}}                                                \\ \hline
					\multicolumn{2}{r}{TYPE:} & \texttt{CHA} \\
					%\multicolumn{2}{r}{ADD:}  & \multicolumn{2}{l}{(\texttt{!CheckTransaction}, 3125, (3125, 3125))} \\
					\multicolumn{2}{r}{UP:}  & (\texttt{IsCoinBase}, 3120) \\
					\multicolumn{2}{r}{DOWN:}  & (\texttt{GetRejectCode}, 3126) \\ 
					\multicolumn{2}{r}{DEL:}  & (\texttt{!CheckTransaction}, 3125, (3125, 3125)) \\
                    \hline
				\end{tabular}%
			}
			\end{adjustbox}
		\end{subtable}
	% \end{minipage}
\end{table}

